CorAl -- Are the point clouds Correctly Aligned?

In robotics perception, numerous tasks rely on point cloud registration. However, currently there is no method that can automatically detect misaligned point clouds reliably and without environment-specific parameters. We propose "CorAl", an alignment quality measure and alignment classifier for point cloud pairs, which facilitates the ability to introspectively assess the performance of registration. CorAl compares the joint and the separate entropy of the two point clouds. The separate entropy provides a measure of the entropy that can be expected to be inherent to the environment. The joint entropy should therefore not be substantially higher if the point clouds are properly aligned. Computing the expected entropy makes the method sensitive also to small alignment errors, which are particularly hard to detect, and applicable in a range of different environments. We found that CorAl is able to detect small alignment errors in previously unseen environments with an accuracy of 95% and achieve a substantial improvement to previous methods.

==> backup/introduction_backuo.tex <==
%Determining if point clouds are correctly aligned is essential to enable robust mobile robotics. Applications such as mapping, scene understanding and sensor calibration are prone to miss alignment of point clouds and requires capability to asses reliability of scan alignment used in the process to avoid devastating failures. Alignment error occurs due to uncompensated motion distortion or wrong convergence in the scan registration.  Our system: ``CorAl'' can detect both these type of errors in real-time, even with small alignment errors. 
%Our method  is well grounded in information theory which and we provide an intuitive formulation of the problem. CorAl measures the difference between the entropy of the merged and separate point clouds and can be used to detect miss alignment. For aligned point clouds, the merged cloud and separate point clouds are similarly blured which provides a measure close to zero. In contrast, merged misaligned point clouds tend to ``blur'' the scene which can be observed by the increase in entropy. The separate point clouds are used to discount for the entropy of the scene. Consequently, the measure provides an absolute understanding of the alignment reliability.\\\\


In order to create safe and efficient mobile robots, introspective capabilities are required to assess and recover from perception failures. Various perception tasks, including localization~\cite{zhang_loam_2014,adolfsson_submap_2019}, scene understanding and sensor calibration~\cite{della_corte_unified_2019}, rely on point cloud registration. However, registration may provide incorrect estimates due to wrong convergence, uncompensated motion distortion, sensor noise or lack of features~\cite{andreasson_incorporating_2017}, potentially causing a system failure or hazard. Consequently, it is essential that the quality of registration is assessed, and unsuccessful attempts are rejected or re-estimated.

In the past, various methods have been proposed to assess the alignment quality of point cloud pairs. One category of methods attempts to provide an uncertainty estimate between point clouds~\cite{David_Landry,bengtsson_robot_2003, nieto_scan-slam_2006,prakhya_closed-form_2015}. However, these methods rely on the assumption that the registration has reached a global maximum -- which may be invalid --  and cannot be used to assess absolute alignment quality.

%perhaps more expli
More recently, Almqvist et al. presented a learning approach to detect misaligned point clouds ~\cite{Almqvist}. A strong classifier was trained based on weaker classifiers derived from common point cloud measures~\cite{rusinkiewicz-2001-fasticp,biber_normal_2003,magnusson-2009-phd,chandran-ramesh_assessing_2007,makadia-2006-fully,silva-2005-ga}.
%~\cite{akai_misalignment_2019,biber_normal_2003, stoyanov_comparative_2013, magnusson-2009-phd}. 
The classifiers were evaluated on two outdoor data sets, and although the combined classifier, as well as some of the individual ones, reach almost 90\,\% classification accuracy for the hardest cases on each data set individually, accuracy dropped to around 80\,\% when cross-evaluating between the data sets.
%The authors reported significantly reduced classification accuracy for all evaluated classifiers when applied to new environments. A key reason for the lack of robustness to environmental changes is that current classifiers do not account for the appearance of the environment and rely heavily on parameter tuning.\\

%Alqvist writes that ``we hope that more specific classifiers will be investigated''.
%Work by  Chandran-Ramesh and Paul Newman ~\cite{chandran-ramesh_assessing_2007} later adopted to pointcloud-pairs by almqvist
%akai_misalignment_2019 detect localization error.
%ICP COVARIANCE Monte Carlo: bengtsson_robot_2003
% closed form ~\cite{nieto_scan-slam_2006}.
% closed formprakhya_closed-form_2015
%useful for pose-graph optimization.
In this paper, we propose ``CorAl'': an accurate and fast  alignment measure and binary classifier for point cloud pairs to bridge the gap in classification performance when the method is applied in new unseen environments without retraining.

% both these type of errors in real-time, even with small alignment errors. CorAl 
Our method is well grounded in information theory and gives an intuitive formulation to the alignment quality problem. CorAl measures the difference between the entropy of the merged and separate point clouds. For well-aligned point clouds, the merged cloud and separate point clouds
have similar entropy %are similarly blured 
and provide a measure close to zero. In contrast, misaligned point clouds tend to ``blur'' the scene which can be observed by an increase in entropy. The separate point clouds are used to discount for the entropy inherent in  the scene. Consequently, the measure provides an absolute understanding of the alignment quality. 





%This work is related to large-scale localization and mapping. THere are multiple essential parts in such system and depending on the application requirements they techniques may vary significantly. Many localization problems are related to finding the alignment between point clouds. If the relative alignment is known, the motion or the location of the robot has been determined. Most systems find the alignment by making assumptions on the quality and relative alignment of point clouds and then deploy well established methods from mathematics to solve the alignment. If any of these assumptions are violated, the localization is likely to fail. For example. Most lidar odometry systems uses the motion of the wheel of the robot to compensate for distortion in the data. based on this correction, local registration methods are used to find the relative alignment. This scenario is likely to introduce two different errors, at least to some extent. The first error is that the motion compensation is inaccurate due to slippage, unsyncronized sensors or noise. This causes the data be inaccurate. The second problem depend on that local registration methods have a limited convergence basin. The registration can fail if the initial alignment is not sufficiently close to the true solution. If the localization algorithms is able to detect occurance of such problems, it can likely also be build to manage and recover from them. Thus making more robust localization systems for robots.

The contribution of this paper is an intuitive and simple measure of the absolute alignment quality between pairs of point clouds based on a relative change in scene entropy. We demonstrate how to use this quality measure to learn to detect misaligned point clouds and how to utilize our tool for manual inspection of alignment quality.
We provide an open source ROS/C++ implementation\footnote{https://github.com/dan11003/CorAl-ScanAlignmentClassification} and make our evaluation available to the community. 

We make the following claims: (i) Our proposed measure provides an absolute understanding of alignment quality by accounting for the expected scene entropy. 
(ii) Our method is highly accurate in %specific environments, 
a wide range of environments and %can even improve adaptation to new unseen environments compared to state-of-the-art alignment classification.
generalizes well to new environments without retraining.





%Fig.~\ref{fig:example_1} 


==> backup/related_work_backup.tex <==
 
Various methods have been used to assess alignment quality. Traditional methods calculate the root mean squared (RMS) point-to-point error, which also is the function that
is minimised by iterative closest point (ICP) registration~\cite{ICP}, or a point-to-distribution~\cite{ndtbiber} distance.
%The minimization is typically stopped when a local minima is found or a maximum number of iterations are reached.
As reported in Almqvist et al.~\cite{Almqvist}, the absolute level of score is sensitive to method parameters, environment and sensing noise. Consequently, they are  are poorly suited for global alignment classification. 

A family of methods attempts to estimate the alignment uncertainty between point cloud pairs. 
Some use Monte Carlo strategies to estimate uncertainty by sampling registrations in a region. This exhaustive search is however unpractical in mobile robotics.
Other attempt to estimate uncertainty in closed form using the Hessian, representing the steepness of the alignment score function around a local minima. These methods assumes correct alignment as they are fundamentally limited by the traditional alignment scores. Consequently, the uncertainty estimation and cannot give an absolute alignment quality. 

Almqvist et al.~\cite{Almqvist} extensively explored building classifiers based on the traditional RMS and Point-to-distribution (P2D) scores. 
The authors also derived a classifier based on Chandran-Ramesh and Newman~\cite{chandran-ramesh_assessing_2007}, which attempts to find suspicious regions in the map, counting planar intersections. The authors proposed AdaBoosting for fusing and improving the individual classifiers. While this did not have a major impact on the classification accuracy, their method reduced parameter sensitivity. %When evaluating the learned classifiers to new environments, RMS and NDT-P2D scored around 50\% accuracy. %While modifying NDT-P2D showed improved performance.
While RMS and L2 classifiers performed on par with random when transferred into new environments without adjusting parameters.
We notice that this limitation inherits from the traditional distance measures.

Liao et al. \cite{fuzzybnb} recently proposed a global registration method representing point clouds as fuzzy sets. The method first attempts to find a consistent clustering by centering clusters at representative locations. A measure that compares the similarity of points distributions around cluster centers is then used to provide a quality assessment in the absence of ground truth. 
Unlike other global registration methods, the quality assessment is used as a stop criteria to end the global search when a coarse alignment is reached. Afterwards, fine tuning is applied to refine this coarse solution and obtain a precise alignment. 
This quality assessment is not sensitive to small misalignment. Accordingly, we categorize this work as coarse alignment quality assessment. In this work we're interested in fine alignment quality assessment.
%%The argument of this quality assessment builds on the robustness of the fuzzy center points. When wil this perform and when will it not?
%As the clustering comes with a high complexity, the method is intractable without downs
Additionally, the method requires at least 50\% overlap between the point clouds which may not be possible in mobile robotic applications. 
Our methods does not require a minimum overlap by operating principle, however we consider point clouds with less than 10\% overlap to provide insufficient evidence to determine alignment quality.\\
%WHy not calculate standard error to determine if there exists evidence for overlap????? 
To the best of our knowledge, there is no method for binary classification of point clouds alignment that performs accurate in real-time and adapts well to new environments.\\

The rest of the paper is structured as follows:
In section \ref{sec:method} we describe our alignment measure and how to train it for binary classification. In section \ref{sec:eval} we propose a benchmark test for further research in the area and evaluate our method on publicly available data.
%https://github.com/zgojcic/3DSmoothNet deep learning high recall
%  Chandran-Ramesh and Paul Newman 

%Introduction
%relative alignment  - local registration
% icp - rms
% ndt - l2 distance
% limited convergence basin - unsuitable for quality assesment
% Broad convergence basin Efficient Global Optimization

%


%Global typically costly, for offline.

%ICP measure%A method for registration of 3-D shapes
%Alqvist et al. \cite{Almqvist} uses AdaBoost to improve a set of weak classifiers.

%Similar covariance estimation}

==> method_backup.tex <==
\label{sec:method}


%We propose measure the quality by determine how the scene is ``blured'' by joining the point clouds.
Our work is inspired by the map quality assessment Mean-Map-Entropy (MME) proposed by Droeschel and Behnke~\cite{8461000}. MME is based on differential entropy~\cite{article} and measures the randomness of multivariate Gaussian distributions. The authors in~\cite{8461000} used the MME score in absence of accurate ground truth when evaluating map refinement.
As shown in our evaluation, MME cannot be used as a direct alignment quality measure as it is impacted by measurement noise, environment geometry and sample density. We instead overcome this effect using dual MME measurements computed 1) in both pointclouds separately and 2) in the aligned pointcloud. \\


%Assuming the point clouds $(\mathcal{P}_a,\mathcal{P}_b)$ given in a common reference frame. %we measure the entropy jointly $H_j$ and separately $H_s$. Our method operates on the relation between these two measurements.\\

The intuition is that joining two well aligned point clouds should not introduce additional uncertainty.
\todo{Insert figure of how a covariance grow as scans are misaligned.}

Typically $Q(\mathcal{P}_a,\mathcal{P}_b)$ is close to zero for well-aligned point clouds and increases with the alignment error as depicted in Fig.~\ref{fig:qualityMeasurePlot}, which visualizes the function's surface for position and angular alignment errors around the correct alignment.
\begin{figure}
[!htp]
\centering
\subfloat[\raggedright CorAl measure with position displacements.]{\includegraphics[trim={0.0cm 0cm 0.0cm 0cm},clip,width=0.49\hsize]{figures/ETH/objective/narrow_position_objective.png}\label{fig:qualitymeasure_wide}}
\subfloat[\raggedright Angular and position displacements.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.49\hsize]{figures/ETH/objective/narrow_angle_objective.png}\label{fig:qualitymeasure_wide}}\hfill \\
\subfloat[Point clouds with alignment quality measured by CorAl.]{\includegraphics[trim={0cm 13cm 0cm 8cm},clip,width=0.99\hsize,angle=0]{figures/stairs2.png}\label{fig:qualitymeasure_wide}}
\caption{\label{fig:qualityMeasurePlot}%Typical values of the quality measure $Q$ for a pair of scans in the ``stairs'' sequence of the ETH registration dataset~\cite{Pomerleau:2012}. The measure consistently provides a global minimum close to 0 around the true position and is sensitive to alignment errors, especially in rotation. These properties enable detection of misaligned point clouds with small errors. }
In these figures we plot the CorAl measure for various alignment offsets ($x,y,\theta$). CorAl has a minimum at the true position(center of figures) with a level consistently close to zero. The steepness of the surface around the true alignment makes the method sensitive to small alignment errors.}
\end{figure}

Well-aligned point clouds $\mathcal{P}_a\cup\mathcal{P}_b$ from structured environments have low entropy for most query points $q_k$. This is reflected by low values for the determinant of the sample covariance. As the determinant can be expressed as the product of the eigenvalues of the sample covariance $|\bold{\Sigma(q_k)}|=\lambda_1\lambda_2\lambda_3$, we see that the score is sensitive to an increase in the lowest of the eigenvalues when larger eigenvalues are constant. For example, the entropy of points on a planar surface is represented with a flat distribution with two large ($\lambda_1,\lambda_2$) and one small($\lambda_3$) eigenvalue. Misalignment changes the point distribution in the registered point cloud from flat to ellipsoidal which can be observed as an increase of the smallest eigenvalue $\lambda_3$. This makes the measure sensitive to misalignment of planar surfaces.
%The effect is further visualized in Fig.~\ref{fig:entropypdf}.

\begin{figure}
\centering
\subfloat[Entropy probability distribution for aligned point clouds. Separate and registered entropy distributions are similar, except at the region between
(${-16}$ and ${-8}$).]{\includegraphics[trim={0.0cm 0cm 0.0cm 0cm},clip,width=\hsize]{figures/aligned_distributions.png}\label{fig:entropy_aligned}}\\
\vspace{-0.1cm}
\subfloat[Probability distribution of misaligned Point Clouds. The distributions are different.]{\includegraphics[trim={0.0cm 0cm 0.0cm 0cm},clip,width=\hsize]{figures/misaligned_distributions.png}\label{fig:entropy_misaligned}}
\caption{\label{fig:entropypdf}Entropy probability distribution for a large amount of aligned and misaligned point clouds with error as defined in Sec.~\ref{sec:benchmark}. Registered and separate entropy are colored in blue and green respectively. Misaligned point clouds shifts the registered entropy distribution to higher entropies. Measurements in the figure are acquired from the dataset in Fig.~\ref{fig:orkla}. }
\end{figure}

Note that the measure in Eq.~\ref{eqn:EntropyDifference} captures discrepancies between point clouds due to rigid or non-rigid distortions, for example, due to slippage or vibrations.

A certain level of overlap is required for the score to be effective as no overlap would provide a zero score; the registered average entropy (Eq.\ref{eq:Hjoint}) would be equal to the separate average entropy (Eq.\ref{eq:Hseparate}). 
\todo{Explain more clearly the role of overlapping and non-overlapping parts, and why that makes sense.}
We have therefore set a minimum overlap ratio of $10\%$. Point clouds with lower overlap are considered not to be aligned.
The quality score is only affected by overlapping segments, hence non overlapping segments between $\mathcal{P}_a$ and $\mathcal{P}_b$ can be removed before applying the quality measure.

%Consider using confidence intervals to obtain a robust minimum overlap.\\


%hence it's sufficient to consider the overlapping subset of all points. % Accordingly, for all points in $\mathcal{P}_a$ we perform a k-d tree search to remove all points without a neighboring point in $\mathcal{P}_b$ within a radius $r$. %Having different densities??
%Accordingly, we perform a filtering step %k-d tree search 
%and keep only the points which has a neighboring point within a radius $r$ in the other point cloud.
%The same radius is used both to determine the overlap and entropy, as described in eq.~\ref{eqn:point_entropy}.% The parameter $r$ has to be selected such that...\\
%Major scene variations can affect the global maxima of $Q(\mathcal{P}_a,\mathcal{P}_b)$. For that reason we further investigated how our measures affect the separability of the aligned and misaligned point clouds. Fig.~\ref{fig:separability} demonstrate this challenge in a structured and an unstructured scenario. 
\subsection{Dynamic radius selection and outlier rejection }
%eally, The CorAl measure in Eq.~\ref{eqn:EntropyDifference} outputs zero for well-aligned point clouds and increase with alignment error. 
It is desired that registered and separate entropy distributions are similar for well-aligned point clouds, and provide a CorAl measure $Q(\mathcal{P}_a,\mathcal{P}_b)=0$.
\todo{Why = 0}
However as seen in Fig.~\ref{fig:entropy_aligned}, differences can be found in the differential entropy distribution.

%the registered entropy increase only for misaligned point clouds and
%While the entropy ideally increases only when register misaligned point clouds, it may also happen for some points in aligned point clouds as seen in Fig.~\ref{fig:entropy_aligned}.
We notice that the majority of this effect can be attributed to a shift of the lowest separate differential entropies. These entropies are measured at solitary point segments, floor segments or when the radius $r$ is small and the neighboring points do not accurately represent the shape of the environment. 

\begin{figure*}[htb!]
  \begin{center}
    \subfloat[\raggedright Fixed radius $r=0.5$ m gives alignment quality $Q_{al}=0.41$ and $Q_{misal}=0.74$]{\includegraphics[trim={0.8cm 1cm 15cm 7cm},clip,height=3.8cm]{figures/failure_case/entropy_1.png}\label{fig:settings_a}}
    \hspace{0.01cm}
    \subfloat[\raggedright$r_{min}=0.2$ m, $r_{max}=1.0$ m, $\alpha = 0.9^{\circ}$ gives alignment quality $Q_{al}=0.2$ and $Q_{misal}=0.46$.  ]{\includegraphics[trim={0.8cm 1cm 15cm 7cm},clip,height=3.8cm]{figures/failure_case/entropy_2.png}\label{fig:settings_b}}
    \hspace{0.01cm}
    \subfloat[\raggedright$r_{min}=0.2$m, $r_{max}=1.0$ m, $\alpha= 0.9^{\circ}$, $E_{rej}=20\%$ gives alignment quality $Q_{al}=0.04$ and $Q_{misal}=0.26$.  ]{\includegraphics[trim={0.8cm 1cm 15cm 7cm},clip,height=3.8cm]{figures/failure_case/entropy_3.png}\label{fig:settings_c}}
    \caption{\label{fig:settings_all} Aligned point clouds with various settings of association radius and outlier rejection. Alignment quality is reported for each example given the aligned and corresponding misaligned point clouds, with error as defined in Sec.~\ref{sec:benchmark}.
    Points with no difference between registered and separate entropy are colored in red, points with a difference larger than $1$ is colored in blue. Solitary point segments typically gives an undesired registered entropy increase.
    Introducing a dynamic radius (b) reduces the significance of this effect, especially at larger distances from the sensor. Outlier rejection (c) removes the final undesired points but also remove additional points.}
  \end{center}
\end{figure*}

%\subfloat[Misaligned Pointclouds]{\includegraphics[trim={15.0cm 0cm 15.0cm 0cm},clip,height=\hsize,angle=270]{figures/failure_case/top_view_failure_case.png}\label{fig:entropy_misaligned}}

To address this we select the radius $r$ depending on the distance $d$ from the sensor.
A small radius is used near the sensor where points are located densely, and a larger radius is used for sparse points at a distance. For that reason we let $r$ increase according to the expected sampling density owed to the sensor angular sampling resolution. We select $r=d \sin(\alpha)$ where $\alpha$ is the vertical resolution of the sensor.

%can be selected according to sensor specifications on vertical angular resolution.
Additionally, we discard points with the $E_{rej}$ percent smallest separate entropies. The effect of these settings is depicted in \cref{fig:settings_all} for a rotating 3d-laser observing a warehouse environment. The aim of the outlier rejection and dynamic radius is to maximize the sensitivity defined as the ratio of quality assessment between misaligned and aligned point clouds: $Q_{misal}/Q_{al}$.
%In fig.~\ref{fig:settings_all}, (a), (b) and (c) had a sensitivity of $0.74/0.41=1.8$, $0.46/0.2=2.3$ and $0.26/0.04=6.5$ for a translation error $5cm$ and angular error of $0.005$ radians. In this case 
The largest improvement can be attributed the outlier rejection.




\subsection{Binary alignment classification}
We use logistic regression as a model for classification, predicting classes(aligned, misaligned) and probability. Probability can be of value in various applications. 
For example, in mobile robotics, it is desired that misaligned point clouds are not accidentally reported as aligned, potentially causing a system failure. In contrast, aligned point clouds classified as misaligned can be discarded and are typically harmless. Probability threshold can hence be set according the the importance of avoiding false positives.
In our evaluation we used the separate and registered entropy $H_s$ and $H_r$ as input variables to the classifier. The The class with highest probability is selected.
